SDP-based bounds for graph partition via extended ADMM

We study two NP-complete graph partition problems, $k$-equipartition problems and graph partition problems with knapsack constraints (GPKC). We introduce tight SDP relaxations with nonnegativity constraints to get lower bounds, the SDP relaxations are solved by an extended alternating direction method of multipliers (ADMM). In this way, we obtain high quality lower bounds for $k$-equipartition on large instances up to $n =1000$ vertices within as few as five minutes and for GPKC problems up to $n=500$ vertices within as little as one hour. On the other hand, interior point methods fail to solve instances from $n=300$ due to memory requirements. We also design heuristics to generate upper bounds from the SDP solutions, giving us tighter upper bounds than other methods proposed in the literature with low computational expense.

==> armbruster_kequi_data.tex <==
graph,n,k,nc2opt,gap_nc2opt,hyperplane2opt,gap_hyp,Armbruster(36hourstimelimit)pbTable5.14,graphfilename
\(U_{500,5}\),500,2,2,0,4,100,2,U500.05
\(U_{500,10}\),500,2,26,0,30,15.38,26,U500.10
\(U_{500,20}\),500,2,178,0,179,0.56,178,U500.20
\(U_{500,40}\),500,2,412,0,412,0,412,U500.40
\(U_{1000,5}\),1000,2,1,0,3,200,1,U1000.05
\(U_{1000,10}\),1000,2,39,0,65,66.67,39,U1000.10
\(U_{1000,20}\),1000,2,242,9.01,303,36.49,222,U1000.20
\(U_{1000,40}\),1000,2,737,0,921,24.97,737,U1000.40
\(G_{124,2.5}\),124,2,13,0,13,0,13,G124.02
\(G_{124,5}\),124,2,63,0,64,1.59,63,G124.04
\(G_{124,10}\),124,2,178,0,179,0.56,178,G124.08
\(G_{124,20}\),124,2,449,0,449,0,449,G124.16
\(G_{250,2.5}\),250,2,30,3.45,30,3.45,29,G250.01
\(G_{250,5}\),250,2,116,1.75,117,2.63,114,G250.02
\(G_{250,10}\),250,2,362,1.4,362,1.4,357,G250.04
\(G_{250,25}\),250,2,831,0.36,832,0.48,828,G250.08
\(G_{500,2.5}\),500,2,52,6.12,52,6.12,49,G500.005
\(G_{500,5}\),500,2,226,3.67,237,8.72,218,G500.01
\(G_{500,10}\),500,2,638,1.92,654,4.47,626,G500.02
\(G_{500,20}\),500,2,1765,1.2,1779,2.01,1744,G500.04
\(G_{1000,2.5}\),1000,2,106,3.92,109,6.86,102,G1000.0025
\(G_{1000,5}\),1000,2,479,6.21,492,9.09,451,G1000.005
\(G_{1000,10}\),1000,2,1404,2.71,1431,4.68,1367,G1000.01
\(G_{1000,20}\),1000,2,3437,1.42,3450,1.8,3389,G1000.02
mesh.138.232,138,2,8,0,8,0,8,mesh.138.232
mesh.148.265,148,2,7,0,7,0,7,mesh.148.265
mesh.274.469,274,2,7,0,7,0,7,mesh.274.469
mesh.70.120,70,2,7,0,7,0,7,mesh.70.120
mesh.74.129,74,2,8,0,8,0,8,mesh.74.129


==> randupcsv.tex <==
%\begin{center}
	\pgfplotstabletypeset[  
		font=\footnotesize,
	multicolumn names, % allows to have multicolumn names
	col sep=comma, % the seperator in our .csv file	
	fixed zerofill,
	fixed,
	display columns/0/.style={int detect,
		column name=$n$, % name of first column
		},  % use siunitx for formatting
	display columns/1/.style={int detect,
		column name=$k$,
		},
	display columns/2/.style={precision=2,
		column name=$lb_{DNN}$,
		},
	display columns/3/.style={string type,
		column name=Vc+2opt,
		},
	display columns/4/.style={
		column name=Gap,
		},
	display columns/5/.style={string type,
		column name=Hyperplane+2opt,
		},
	display columns/6/.style={
		column name=Gap,
		},
	every row no 6/.style={before row={\midrule}},
	every row no 11/.style={after row={\midrule
		$\vdots$	&$\vdots$  &$\vdots$  &$\vdots$ &$\vdots$ &$\vdots$  &$\vdots$ \\}},
	every row no 12/.style={before row={\midrule}},
%	every row no 13/.style={before row={\midrule}},
	every row no 20/.style={before row={\midrule}},
	every head row/.style={
		before row={
			\caption{Feasible solutions for randomly generated graph rand80 (for instances with $n=100,200$, the time limit is 1 second; for instances with $n = 900, 1000$, the limit is 3 seconds)}\label{tab:kequi-gap}\\
			\midrule}, % have a rule at top
		after row={
		 &  &  & &\si{\percent} &  &\si{\percent} \\
		  	\midrule} % rule under units
	},	
	every last row/.style={after row=\bottomrule}, % rule at bottom
		]{rand_keq_lb_up_gap.csv} % filename/path to file
%\end{center}



==> randupcsv_20.tex <==
%\begin{center}
	\pgfplotstabletypeset[  
		font=\footnotesize,
	multicolumn names, % allows to have multicolumn names
	col sep=comma, % the seperator in our .csv file	
	fixed zerofill,
	fixed,
	display columns/0/.style={int detect,
		column name=$n$, % name of first column
		},  % use siunitx for formatting
	display columns/1/.style={int detect,
		column name=$k$,
		},
	display columns/2/.style={precision=2,fixed zerofill,
		column name=$lb_{DNN}$,
		},
	display columns/3/.style={string type,
		column name=Vc+2opt,
		},
	display columns/4/.style={
		column name=Gap,fixed zerofill
		},
	display columns/5/.style={string type,
		column name=Hyperplane+2opt,
		},
	display columns/6/.style={
		column name=Gap,fixed zerofill
		},
	every row no 6/.style={before row={\midrule}},
	every row no 11/.style={after row={\midrule
			$\vdots$	&$\vdots$  &$\vdots$  &$\vdots$ &$\vdots$ &$\vdots$  &$\vdots$ \\}},
	every row no 12/.style={before row={\midrule}},
	every row no 20/.style={before row={\midrule}},
	every head row/.style={
		before row={
		\caption{Feasible solutions for randomly generated graph rand20 (for instances with $n=100,200$, the time limit is 1 second; for instances with $n = 900, 1000$, the limit is 3 seconds)}\label{tab:kequi-gap-20}\\
			\midrule}, % have a rule at top
		after row={
		 &  &  & &\si{\percent} &  &\si{\percent} \\
		  	\midrule} % rule under units
	},	
	every last row/.style={after row=\bottomrule}, % rule at bottom
		]{rand_keq_lb_up_gap_20.csv} % filename/path to file
%\end{center}

==> randupcsv_50.tex <==
%\begin{center}

	\pgfplotstabletypeset[  
		font=\footnotesize,
	multicolumn names, % allows to have multicolumn names
	col sep=comma, % the seperator in our .csv file	
	fixed zerofill,
	display columns/0/.style={int detect,
		column name=$n$, % name of first column
		},  % use siunitx for formatting
	display columns/1/.style={int detect,
		column name=$k$,
		},
	display columns/2/.style={precision=2,fixed,
		column name=$lb_{DNN}$,
		},
	display columns/3/.style={string type,
		column name=Vc+2opt,
		},
	display columns/4/.style={precision=2,fixed,
		column name=Gap,
		},
	display columns/5/.style={string type,
		column name=Hyperplane+2opt,
		},
	display columns/6/.style={precision=2,fixed,
		column name=Gap,
		},
	every row no 6/.style={before row={\midrule}},
	every row no 11/.style={after row={\midrule
			$\vdots$	&$\vdots$  &$\vdots$  &$\vdots$ &$\vdots$ &$\vdots$  &$\vdots$ \\}},
	every row no 12/.style={before row={\midrule}},
	every row no 20/.style={before row={\midrule}},
	every head row/.style={
		before row={
			\caption{Feasible solutions for randomly generated graph rand50 (for instances with $n=100,200$, the time limit is 1 second; for instances with $n = 900, 1000$, the limit is 3 seconds)}\label{tab:kequi-gap-50}\\
			\toprule}, % have a rule at top
		after row={
		 &  &  & &\si{\percent} &  &\si{\percent} \\
		  	\midrule} % rule under units
	},	
	every last row/.style={after row=\bottomrule}, % rule at bottom
		]{rand_keq_lb_up_gap_50.csv} % filename/path to file
%\end{center}
